Accelerating HEP simulations with Neural Importance Sampling

Many high-energy-physics (HEP) simulations for the LHC rely on Monte Carlo using importance sampling by means of the VEGAS algorithm. However, complex high-precision calculations have become a challenge for the standard toolbox, as this approach suffers from poor performance in complex cases. As a result, there has been keen interest in HEP for modern machine learning to power adaptive sampling. While previous studies have shown the potential of normalizing-flow-powered neural importance sampling (NIS) over VEGAS, there remains a gap in accessible tools tailored for non-experts. In response, we introduce Z\"uNIS, a fully automated NIS library designed to bridge this divide, while at the same time providing the infrastructure to customise the algorithm for dealing with challenging tasks. After a general introduction on NIS, we first show how to extend the original formulation of NIS to reuse samples over multiple gradient steps while guaranteeing a stable training, yielding a significant improvement for slow functions. Next, we introduce the structure of the library, which can be used by non-experts with minimal effort and is extensivly documented, which is crucial to become a mature tool for the wider HEP public. We present systematic benchmark results on both toy and physics examples, and stress the benefit of providing different survey strategies, which allows higher performance in challenging cases. We show that Z\"uNIS shows high performance on a range of problems with limited fine-tuning.

==> introduction/coupling_cell_figure.tex <==
\begin{figure}
\centering
\resizebox{\textwidth}{!}{%
\tikzstyle{init} = [pin edge={to-,thin,black}]
\begin{tikzpicture}[cn/.style={circle, fill=white,  thick,draw=black, minimum size=4cm},txt/.style={},d/.style={circle, fill=white,  thick,draw=black, minimum size=0.5cm},d2/.style={circle, fill=white,  thick,draw=black, minimum size=1cm},d3/.style={circle, fill=white,  thick,draw=black, minimum size=1cm}, box/.style={rectangle, fill=magenta!10!blue!10,very thick, draw=magenta!20!blue!20, minimum size=5cm},sbox/.style={rectangle, fill=magenta!20!blue!15,very thick, draw=magenta!40!blue!30, minimum size=1.5cm},s2box/.style={rectangle, fill=magenta!15!blue!20,very thick, draw=magenta!30!blue!40, minimum size=1cm},box2/.style={rectangle, fill=magenta!10!blue!10,very thick, draw=magenta!20!blue!20, minimum height=5cm, minimum width=1cm},d4/.style={circle, fill=white,  thick,draw=white, minimum size=0.5cm},]
\node[d3,label={[label distance=0.2cm]100:Masking}] (c) at (-3.5,0) {};
\node[box, label=above:Coupling cell 1] (b) at (0,0) {} ;
\node[sbox] (sb) at (1,0.2) {$m(x^A)$};
\node[s2box] (ssb) at (1,-1.8) {$C(x^B;m(x^A))$};
\node[box2, label=above:Coupling cell 2] (b2) at (5,0) {};

\node[d4] (txt1) at (6.5,0) {$\dots$};
\node[d3] (c2) at (10,0) {};
 
\draw[ultra thick, draw=blue!50] (-4.2,0) node[above] {$x$} -- (-3.5,0) ;
\draw[ultra thick, draw=blue!50] (-3.5,0) -- (-2.8,1.8) node[above] {$x_A$};
\draw[ultra thick, draw=blue!50] (-3.5,0) -- (-2.8,-1.8) node[below] {$x_B$};
\draw[ultra thick, draw=blue!50] (-2.8,-1.8) -- (ssb.west);
\draw[ultra thick, draw=blue!50] (-2.8,1.8) -- (2.6,1.8) node[right] {$y_A$};
\draw[ultra thick, draw=blue!50] (ssb.east) -- (2.6,-1.8) ;
\draw[ultra thick, draw=blue!50] (1,1.8) -- (sb.north);
\draw[ultra thick, draw=blue!50] (2.6,1.8)  -- (3.5,0);
\draw[ultra thick, draw=blue!50,->] (sb.south) -- (ssb.north);
\draw[ultra thick, draw=blue!50] (2.6,-1.8) node[right] {$y_B$} -- (3.5,0);
\draw[ultra thick, draw=blue!50] (3.5,0) -- (4.4,1.8);
\draw[ultra thick, draw=blue!50] (3.5,0) -- (4.4,-1.8);
\draw[ultra thick, draw=blue!50, dashed] (4.4,-1.8) -- (5,-1.8);
\draw[ultra thick, draw=blue!50,dashed] (4.4,1.8) -- (5,1.8);
\node[box2, label=above:Coupling cell $n$] (bn) at (8,0) {};
\draw[ultra thick, draw=blue!50, dashed] (8,-1.8) -- (8.5,-1.8);
\draw[ultra thick, draw=blue!50,dashed] (8,1.8) -- (8.5,1.8);
\draw[ultra thick, draw=blue!50] (8.5,-1.8) -- (10,0);
\draw[ultra thick, draw=blue!50] (8.5,1.8) -- (10,0);
\draw[ultra thick, draw=blue!50,->] (10,0) -- (11.5,0) node[above] {$z$};
\draw[ultra thick, draw=red!50] (-4.2,-3)node[left] {$\Pi$} -- (1,-3);
\draw[ultra thick, draw=red!50] (ssb.south) -- (1,-3) node[below] {$J_1$};
\draw[ultra thick, draw=red!50] (1,-3) -- (5,-3);
\draw[ultra thick, draw=red!50] (b2.south) -- (5,-3) node[below] {$J_2$};
\draw[ultra thick, draw=red!50] (5,-3) -- (8,-3);
\draw[ultra thick, draw=red!50] (bn.south) -- (8,-3) node[below] {$J_n$};
\draw[ultra thick, draw=red!50, ->] (8,-3) -- (11,-3) node[right] {$\Pi_{i=1} ^n J_i$};
\end{tikzpicture}
}
    \caption{Schematic structure of a coupling layer.}
    \label{fig:cl}
\end{figure}

==> introduction/related_works.tex <==
Importance sampling requires, as mentioned before, to learn a probability distribution and to sample from the learned model, which is called generative modeling. We review the most common generative neural network approaches in the context of MC integrations and applications for high energy physics. \\

Deep Boltzmann machines \cite{salakhutdinov2008quantitative,salakhutdinov2009deep} can quickly learn distributions, but are very costly in sampling due to the requirement of using Markov chain Monte Carlo procedures, which also limits the applicability for sharp modes in the distributions.
Independent component analysis \cite {hyvarinen2000independent} attempts to learn the probability distribution by decomposing it into orthogonal component distributions. This, however, requires to perform a costly orthogonalization procedure at every parameter update. Generalizations of this approach exist \cite{bengio1993artificial,chen2000gaussianization,rippel2013highdimensional,hyvarinen1999nonlinear,roberts2001independent}, but the inference is in general not satisfying.
Variational auto-encoders (VAEs)\cite{kingma2013auto,rezende2014stochastic,mnih2014neural,gregor2014deep} are an alternative approach, consisting of an stochastic encoder $q(u|x)$ and an imperfect decoder $p(x|u)$, such hat the loss consists of an reconstruction term . This trains the model in such a way that the decoder approximately inverts the encoder. VAEs allow fast sampling and give access to the inverse of the model, but are prone to noise due to the imperfect inverse. Additionally, many VAEs rely on auxiliary latent variables $z$ with fixed PDFs $q(z)$, so that the the distribution becomes $q(x|z;h)$ which is learnable via the parameters $h$. Now the same $x$ can be caused by multiple $z$. In order to have access to $q(x|h)$, which is necessary for importance sampling, one has to integrate over $z$ which causes significant additional computational cost. 
Generative adversary networks (GANs) avoid the encoder and only train a generative model to transform a distribution into the data distribution  \cite{goodfellow2014generative}. This is a achieved by training a secondary neural network to discriminate between the training data and the generated data. The classifier is then used to determine the training success. They suffer from the disadvantage that, though sampling is possible, the PDF $q$ cannot be directly evaluated, which is a major downside for the application to MC integration.\\

The advantage of normalizing flows is that they are a deterministic bijective mapping of $u\rightarrow x=h(u;\theta)$. Other than for generative models where multiple $u$ are assigned to the same $x$ (like for VAEs), one can avoid integration over a PDF for $u$. The only requirement for this to be efficient for MC integration  is to have a tractable inverse and a fast evaluation, in order to know the correspondence between $u$ and $x$.  Several prior works on normalising flows tried to achieve this.
Normalizing flows have been used in complex computation graphs for learning distributions \cite{rezende2015variational}, which however doesn't permit an easy inversion of mapping. A possible solution to improve the computational cost of the inversion and the calculation of the Jacobian was proposed by introducing continuous normalizing flows \cite{chen2019neural}. They only need a computation of the trace of the Jacobian instead of the determinant, at the cost of introducing a numeric ODE solver, which both affects performance and introduces approximation errors and possibly leads to bias in MC integration.
Multiple recent approaches use normalizing flows for auto-regressive density estimations like masked auto-regressive flows (MAF) \cite{kingma2016improving,huang2018neural,papamakarios2017masked}. This is inspired from neural auto-regressive networks \cite{bengio2000modeling} like the neural auto-regressive density estimator (NADE) \cite{larochelle2011neural}, for which the adjacency matrix is strictly triangular, but lacks the coupling cell structure which makes it computationally expensive for high-dimensional data. Auto-regressive flows combine the approach with normalizing flows and decompose a joint distribution over $d$-dimension in a product of univariate conditionals. This largely reduces the computational cost when calculating the Jacobian, as it can be now computed with linear cost. However, these approaches cannot generate data and estimate densities at the same time, which disqualify them for our use case. 
Our approach follows instead the direction of by non-linear independent components estimation (NICE) \cite{dinh2014nice, dinh2016density}.  Although NICE and its extension Real NVP (real-valued non-volume preserving transformations) can be seen as less flexible predecessors of MAF and others, with which they share the concept of coupling cells, they are suited best for MC integration as they allow simultaneously fast sampling and density evaluation without requiring approximations. NICE can be seen as an ideal auto-encoder, as the transformation and its inverse are a perfect encoder-decoder pair.
The transformations used in Real NVP were generalised to quadratic coupling layers and applied to MC integration \cite{mller2018neural, durkan2019neural}. Convolutions can be also included \cite{kingma2018glow}, which is especially relevant for image generation.\\

The improvements in the field of generative models were also used in high-energy physics for improvement of MC integration of matrix elements. Machine learning was used first in the context of high-energy physics in the form of boosted decision trees, GANs and dense neural networks, which improved the integration of non-separable high dimensional functions \cite{bendavid2017efficient} and could also show considerable improvements for phase space integration when applying them to learn the phase space directly \cite{klimek2018neural}, but suffer from the mentioned disadvantages of the high cost of inverting neural networks.  
A conceptionally different technique in speeding up the integration of cross sections is the replacement of the exact amplitudes used in MC event generators by trained Machine Learning regressors \cite{hashemi2019lhc, Ahdida_2019, Di_Sipio_2019,Carrazza_2019,Butter_2019, bishara2020machine, Badger_2020, Nachman_2020,Butter_2020, otten2021event}. While these approaches report drastic improvements of runtime,  they require a considerable number of pre-generated events for training. Especially for high-multiplicity events, this can be a great disadvantage. Additionally, such methods can only generate events similiar to such which were used during training. Too small training sets would result then into a bias which ignores corners of distributions and result in incorrect cross sections. 
Another recent approach using normalizing flows in generative models for high energy physics are generative models for Markov chain Monte Carlo (MCMC) in lattice field theory \cite{Albergo_2019,Kanwar_2020,albergo2021introduction}.  Other than earlier machine learning approaches for MCMC like Self-Learning Monte Carlo \cite{huang2017accelerated,nagai2017self}, this does not aim at learning an effective Hamiltonian which is easier to sample from, but instead on generating samples from a good approximation of the underlying distribution.  The samples are then used in lattice frameworks to estimate expectation values of observables. Normalizing flows proved to be very successfull when designed in such a way that they are gauge-invariant. Under this condition, they show to perform well in cases in which conventional algorithms suffer from critical slowing down. Essential for the application of this method in general gauge theories was also the generalisation of normalizing flows to tori ans spheres \cite{rezende2020normalizing}. An overview of existing approaches, not just for phase space generation but for generative networks for LHC events in general, is given in recent reviews \cite{Bourilkov_2019, butter2020generative}.\\

Normalizing flows similiar to our approach are used in \textsc{i-flow} \cite{Gao_2020,Gao_20202}, which implements the coupling layers with multiple different transformations in Tensorflow instead of \textsc{PyTorch} in the present implementation. \textsc{i-flow} provides a choice of different loss functions and forms of the NN, but provides less options in how the training is performed.




==> performance/madgraph.tex <==
As the \zunis package does not require any specific form of the integrand, it can be easily used together with a phase space generator and a process generator in order to increase the precision of cross section integration.

Cross-sections are integrals of matrix elements of a process over the phase-space of the final state particles. The matrix elements can be seen as a probability distribution in the final state phase space, giving the probability of process to happen depending on the momenta of the produced particles. Matrix elements are challenging to integrate, as the presence of divergences require phase space cuts. Additionally, processes involving initial state partons require parton distribution functions (PDFs), which can induce correlations amongst the integration variables. \zunis can learn the probability distribution efficiently and use it to perform importance sampling. An example of this is included in the Github repository.

In the following, we want to study the performance of \zunis in comparison to \textsc{VEGAS} by studying the integration of three standard processes, $ e^- \mu \rightarrow e^- \mu$ via $Z$, $ d \bar d \rightarrow d \bar d$ via $Z$ and $ u c \rightarrow u c g$.  The aim is to test the performance in comparison to \textsc{VEGAS} both for rather simple processes as well as for processes involving parton density functions and higher multiplicities. We show that the improvement in evaluation time needed to reach a certain precision in comparison to \textsc{VEGAS} is considerable, as can be seen in \cref{tab:eval}.

\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|S[table-format=3.5(2 ),table-figures-exponent = 0]|S[table-format=4.5(2 ),table-figures-exponent = 0]|S[table-format=5.4(2 ),table-figures-exponent = 0]|}
\hline
    \multicolumn{2}{|c|}{Precision/process} & \text{ $ e^- \mu \rightarrow e^- \mu$ via $Z$ }&\text{$ d \bar d \rightarrow d \bar d$ via $Z$} &\text{$ u c \rightarrow u c g$}\\
    \hline
    \hline
   
  \multirow{4}{*}{10\% rel. error} & \#1& 0.04612(74) &0.0730(74) &0.338(11) \\ \cline{2-5} 
   & \#2& 0.0496(21) &0.05972(77) & 0.543(57)\\ \cline{2-5} 
   & \#3& 0.0499(15) &0.0757(67) &  0.468(29)\\ \cline{2-5} 
  & \textsc{VEGAS}& 0.2001(27) &0.333(18) & 1.1434(41) \\\hline
  \multirow{4}{*}{1\% rel. error} & \#1& 0.307(13) &1.26(57) & 4.077(19)\\ \cline{2-5} 
   & \#2& 0.309(13) &0.88(10) & 6.19(99)\\ \cline{2-5} 
   & \#3& 0.317(12) &1.61(55) & 5.18(72) \\ \cline{2-5} 
  & \textsc{VEGAS}& 1.285(18)&15.98(57) & 95.48(98)\\\hline
  \multirow{4}{*}{0.1\% rel. error} & \#1& 8.3(22) &120(54) & 435(63) \\ \cline{2-5} 
   & \#2& 10.1(21) &79.2(95)& 633(103)\\ \cline{2-5} 
   & \#3& 6.21(45) &165(56) & 455(100) \\ \cline{2-5} 
  & \textsc{VEGAS}& 55.31(90) &1526(59) & 12601(990)\\\hline
  
  \hline
\end{tabular}}
\label{tab:eval}
\caption{Comparison of the average evaluation times in seconds over all trained models.}
\end{table}
In order to do so, one has to generate the matrix element. In the example, this is done by interfacing \textsc{MadGraph5\_aMC@NLO} \cite{madgraph}. \textsc{MadGraph} generates matrix elements for a specific process as a \textsc{Fortran} executable, which can be evaluated during the survey/refine phase given the four-momenta of the final state particles.  Although the evaluation of the integrand is due to this still performed on CPU, the sampling can be executed efficiently on GPU. The PDFs are provided by interfacing  LHAPDF6 \cite{lhapdf}.

\subsubsection{Phase space sampling}
\zunis samples into the hypercube, whereas a phase space integral is an integral over $\mathbb{R}^{3n-4}$, with $n$ the number of final state particles, which can be written like
\begin{equation}
  \diff\phi_n(\{p_1,m_1\},\dots,\{p_n,m_n\}|Q)=\delta \left(\sum_{i=1}^n p_n-Q\right)\Pi_{i=1}^n \diff^4 p_i \delta(p_i^2-m_i^2)\theta(p_i^0-m_i)
\end{equation}
where the total momentum is $Q$ and the $p_i$ are the final state 4-vectors of particles with mass $m_i$. It is necessary to map the hypercube into the phase space in such a way that the kinematic conservation laws are respected (like momentum conservation), but at the same time the phase space should be covered evenly, in order to not induce as less additional variance as possible.  

This can be done by using the "RAMBO on diet" algorithm \cite{pltzer2013rambo}. The starting point is the decomposition of the multiparticle phase space with final states $\{p_i,m_i\}$ into subsequent $1\rightarrow 2$ decays with intermediate states $\{Q_i,M_i\}$ 
\begin{equation}
\begin{split}
    \diff\phi_n(\{p_1,m_1\},\dots,\{p_n,m_n\}|Q)&=
    \left(\prod_{i=2}^n \diff \phi_2 (\{p_{i-1},m_{i-1}\},\{Q_i, M_i\}|Q_{i-1})\right)\\\cdot&
    \left(\prod_{i=2}^n \theta(M_{i-1}-m_{i-1}-M_i) \theta\left(M_i-\sum_{k=i}^n m_k\right)\diff M_i^2\right)
    \label{equ:phin}
\end{split}
\end{equation}
with $Q_1=Q$ and $\{Q_n,M_n\}=\{p_n,m_n\}$ and without prefactors. Now, each of the two particle phase spaces can be expressed in the rest frame of its mother particle:
\begin{equation}
    \diff\phi_2(\{p_{i-1},m_{i-1}\},\{Q_i, M_i\}|Q_{i-1})=\rho (M_{i-1},M_i,m_{i-1})\diff\cos\theta_{i-1}\diff\phi_{i-1}.
\end{equation}
Here, $\rho$ is a weight that comes from the requirement of being on-shell:
\begin{equation}
\begin{split}
    &\mathbf{p}_{i-1}= -\mathbf{Q_i}= 4M_{i-1}\rho (M_{i-1},M_i,m_{i-1})(\cos\phi_{i-1}\sin\theta_{i-1}, \sin\phi_{i-1}\sin\theta_{i-1},\cos\theta_{i-1})^T \\
    & \rho=\frac{1}{8M_{i-1}^2}\sqrt{\left(M_{i-1}^2-(M_i-m_{i-1})^2\right)+\left(M_{i-1}^2-(M_i+m_{i-1})^2\right)}
\end{split}
\end{equation}
The zero-component can be then deduced from the on-shellness condition. The resulting final-state momenta can be brought into the centre-of-mass frame by a Lorentz boost, which preserves flatness. The flatness of the phase space generation is, when the angles are sampled in such a way that isotropy is guaranteed, only dependent on the sampling of the intermediate masses. This can be achieved by sampling them proportional to the measure of the two body phase spaces:
\begin{equation}
\begin{split}
     &\diff M_n(M_2,\dots,M_{n-1}|M_1;m_1,\dots,m_n)=\\&\rho(M_{n-1},m_n,m_{n-1})\\&\cdot\left(\prod_{i=2}^n \rho (M_{i-1},M_i,m_{i-1})\theta(M_{i-1}-m_{i-1}-M_i) \theta\left(M_i-\sum_{k=i}^n m_k\right)\diff M_i^2\right)
 \end{split}
 \label{equ:M}
\end{equation}
where $M_1$ is the mass of the initial state.

In the case of massless final states, this can be written as
\begin{equation}
    \diff M_n(M_2, \dots, M_{n-1}|M_1;0,\dots,0)=\frac{1}{8^{n-1}}\prod_{i=1}^{n-1}\frac{M^2_{i-1}-M_i^2}{M^2_{i-1}}\theta(M_{i-1}^2-M_i^2)\theta(M_i^2)\diff M_i^2
\end{equation}
It is always possible to write $M_i=u_2\dots u_i M_{1}$. The $u_i$ can be seen as the ratios of centre-of-mass energy being carried forward to the next decay at each step. Thus one gets
\begin{equation}
    \diff M_n(M_2, \dots, M_{n-1}|M_1;0,\dots,0)=\frac{1}{8^{n-1}}M_1^{2n-4}\prod_{i=1}^{n-1} u_i^{n-1-i}(1-u_i)\theta(1-u_i)\theta(u_i)\diff u_i
    \label{eq:ra}
\end{equation}
Using $v_i=(n+1-i)u^{n-i}_i-(n-i)u_i^{n+1-i}$, this can be expressed as
\begin{equation}
\begin{split}
    \diff M_n(M_2, \dots, M_{n-1}|M_1;0,\dots,0)&=\\ &=\frac{1}{8^{n-1}}M_1^{2n-4}\frac{1}{(n-1)!(n-2)!}\prod_{i=1}^{n-1} \theta(1-v_i)\theta(v_i)\diff v_i
\end{split}
\end{equation}
Starting from this description, it is possible to define an algorithm which performs a mapping from $[0,1]^{3n-4}$ into the flat massless $n$-particle phase space, which is the desired result. 
\begin{algorithm}[H]
\SetAlgoLined
\KwData{random numbers $r_0, \dots, r_{3n-4}, Q_1=E_{cm}, M_1=E_{cm}, M_n=0$}
\KwResult{Flat sampled momenta $\{p_1,\dots,p_n\}$ with weight $V_n$}
 
 \For{$i=2,\dots, n-1$}{
  solve $r_{i-1}=v_i=(n+1-i)u^{n-i}_i-(n-i)u_i^{n+1-i}$ for $u_i$\;
  $M_{i}\leftarrow u_2\dots u_i M_1$\;
  $\cos \theta_i \leftarrow 2r_{n-5+2i}-1, \phi_i\leftarrow 2\pi r_{n-4+2i}$\;
  $q_{i-1} \leftarrow 4 M_{i-1}\rho(M_{i-1},M_i,0)$\;
  $\sin\theta_{i-1}\leftarrow \sqrt{1-\cos \theta_{i-1}}$\;
  $\mathbf{p}_{i-1}= 4M_{i-1}\rho (M_{i-1},M_i,m_{i-1})(\cos\phi_{i-1}\sin\theta_{i-1}, \sin\phi_{i-1}\sin\theta_{i-1},\cos\theta_{i-1})^T $\;
  $p_{i-1}\leftarrow(q_{i-1},\mathbf{p}_{i-1})$,$Q_i\leftarrow (\sqrt{q_{i-1}^2+M_i^2},-\mathbf{p}_i)$\;
  boost $p_i$ and $Q_i$ by $\mathbf{Q}_{i-1}/Q_{i-1}^0$\;
 }
 $p_n\leftarrow Q_n$\;
 \caption{RAMBO on diet in the massless case}
\end{algorithm}
This algorithm can be further generalised to the massive case, for which it is only approximately flat.

In the example at hand, the phase space sampling was performed using the package \textsc{TorchPS} \cite{niklas_gotz_2021_4639109}. The package is also implemented in \textsc{PyTorch}, so that the phase space sampling can directly take the GPU-vectors sampled by \zunis and convert them into phase space points without a significant loss of performance.


\subsubsection{Results}

Using this setup, the advantage of \zunis over \textsc{VEGAS} becomes evident when comparing the evaluation time spent in order to reach a certain level of precision. Though the model is more expensive to sample from than the \textsc{VEGAS} grid, the reduced number of the costly evaluations of  the integrand compensates this as well as the increased training time when aiming for a high precision.

Table \cref{tab:eval} shows the evaluation time for three pre-trained models selected from the winners of hyperparameter optimisation. It becomes clear that, although the chosen hyperparameter optimization does not succeed to consistently find the optimal model but rather hints which parameter combinations are more promising, \zunis performs generally considerably better than VEGAS. For all processes and precision bound, the trained \zunis model reaches the requested precision level considerably faster.  The values were taken by integrating with 20 independently trained copies of the same model in order to account for varying training success of \zunis. Of course, the reported times can be improved by testing the training success and only integrating with the copies which trained the best. This in turn would not just improve the evaluation times but also reduce their standard deviation.


\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|S[table-format=2.2(2 ),table-figures-exponent = 0]|S[table-format=2.2(2 ),table-figures-exponent = 0]|S[table-format=2.2(2 ),table-figures-exponent = 0]|}
\hline
    \multicolumn{2}{|c|}{Result/Process} &  \text{$ e^- \mu \rightarrow e^- \mu$ via $Z$}&\text{$ d \bar d \rightarrow d \bar d$ via $Z$}&\text{$u c \rightarrow u c g$}\\
   \hline \hline
  \multirow{3}{*}{Relative variance reduction}&\#1 &10.9(57) & 31(31)&25(39)\\ \cline{2-5}
  &\#2 & 12.1 (57)& 16(12)&55 (48)\\ \cline{2-5}
  &\#3 & 11.2(55)& 27(26)&51(49)\\ \hline
  \multirow{3}{*}{Relative duration}&\#1 &2.69(32)  & 2.05(68)&1.8(10)\\ \cline{2-5}
  &\#2 &3.38(38) & 2.50(46) &3.29(21)\\ \cline{2-5}
  &\#3 & 2.82(17)& 2.37(68)&3.15(19)\\ \hline
  \hline
  \multirow{3}{*}{Relative improvement}&\#1 & 2.01(91)&3.9(26) &3.7(41)\\ \cline{2-5}
  &\#2 & 1.89(80)& 2.5(14)&4.1(19)\\ \cline{2-5}
  &\#3 & 1.99(78)& 3.4(23)&4.0(20)\\ \hline
  
\end{tabular}}
\label{tab:vardur}
\caption{Average variance reduction, training/integration duration and improvement on a batch of 100.000 points relative to \textsc{VEGAS}.}
\end{table}

Table \cref{tab:vardur} shows, on the other hand, the average performance of all selected configurations for the three processes when training and integration is performed on a fixed number of points. The values are averaged over 100 independently trained models each. Although the duration is considerably increased in comparison to the benchmark, so is the improvement in comparison to flat sampling. All models reach a variance of the integrand after the training of less than a tenth than after training with \textsc{VEGAS}. The variance of the training success is however significant between runs. Nevertheless, depending on the configuration 82-90\% of the models achieve better variance reduction than the benchmark.

The relative improvement factor, representing the factor of time which can be saved by \zunis in comparison to \textsc{VEGAS} is calculated under the assumption that the duration grows linear with the number of sampled points. As the integration error for MC integration is inversely proportional to the square root of evaluation points, the improvement can be calculated as
\begin{equation}
    f_i=\frac{\bar f_\sigma}{\sqrt{\bar f_t}}
\end{equation}
where $\bar f_\sigma$ is the average relative reduction of the standard error, which can be calculated from the relative variance reduction, and $\bar f_t$ is the average relative duration. The improvement factors show that the selected configurations are virtually always superior to \textsc{VEGAS}. Additionally, once a model has been trained, it can be reused, which reduces the improves the integration speed. Again, selecting the trained models for the ones with the greatest improvements can improve the performance.

\subsubsection{Hyperparameter optimisation}
\begin{table}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
    \multirow{2}{*}{Parameter/configuration} &  \multicolumn{3}{c|} {$e^- \mu \rightarrow e^- \mu$ via $Z$}& \multicolumn{3}{c|} {$ d \bar d \rightarrow d \bar d$ via $Z$ }& \multicolumn{3}{c|} {$ u c \rightarrow u c g$}\\
    \cline{2-10}
     &1st&2nd&3rd&1st&2nd&3rd&1st&2nd&3rd\\
    \hline
    \hline
  learning rate &0.005&0.0005&0.001  & 0.01&0.0005&0.005& 0.01&0.0001&0.001\\
  \hline
  number of bins & \multicolumn{3}{c|}{10}&25&5&25&5&5&10\\
  \hline
  number of hidden layers & 2&4&4 & 2&4&4 & 2&4&2 \\
  \hline
  size of hidden layers & 64&128&64 & 64&128&64 & 64&128&128\\
  \hline
  survey strategy &\multicolumn{9}{c|}{adaptive DKL}\\
  \hline
  \hline
  cost & 2.39E-2&2.55E-2&2.58E-2& 1.00&1.32&1.33&4.36E12&1.26E14&1.34E14\\
  \hline
\end{tabular}
}
\label{tab:madgraph_config}
\caption{Chosen configurations for the three processes.}
\end{table}

The three configurations used for each of the processes are listed in \cref{tab:madgraph_config}. They were chosen based on a hyperparameter optimisation. We will outline here how this hyperparameter optimisation was performed, and what values for the parameters represent a reasonable choice.

In a first step, it is necessary to get an understanding of the influence of the hyperparameters on the quality of the trained model. For this, the model is trained with different hyperparameter configurations and the standard deviation of the integral is compared after integration on a fixed sample size, similiar to how the values in \cref{tab:vardur} were derived.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{performance/emu_emu_var_d_hidden.png}
    \includegraphics[width=0.45\textwidth]{performance/emu_emu_var_lr.png}
    \includegraphics[width=0.45\textwidth]{performance/emu_emu_var_n_bin.png}
    \includegraphics[width=0.45\textwidth]{performance/emu_emu_var_n_hidden.png}
    \caption{The relative variance in comparison to \textsc{VEGAS} when varying different hyperparameters for $ e^- \mu \rightarrow e^- \mu$ via $Z$.  }
    \label{fig:em1}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{performance/emu_emu_time_d_hidden.png}
    \includegraphics[width=0.45\textwidth]{performance/emu_emu_time_lr.png}
    \includegraphics[width=0.45\textwidth]{performance/emu_emu_time_n_bin.png}
    \includegraphics[width=0.45\textwidth]{performance/emu_emu_time_n_hidden.png}
    \caption{The relative time consumption in comparison to \textsc{VEGAS} when varying different hyperparameters for $ e^- \mu \rightarrow e^- \mu$ via $Z$.}
    \label{fig:em2}
\end{figure}
From \cref{fig:em1} one can see that there is a strong peak of the training success for the learning rate, whereas other parameters have no (like the number of bins and hidden layers) or only a weak correlation (like the size of the hidden layers) with the training success. It is also noteworthy that in general the adaptive DKL training mode achieves better results. From \cref{fig:em2} on the other hand, one can see that the number of bins has a strong effect on the training time due to the increased cost of sampling from the model, whereas the increased cost due to the more and wider linear layers is less significant. The other processes show similiar correlations. Therefore, hyperparameter optimisation is best for a wide range of the learning rate to find the peak, and smaller ranges for the other hyperparameters with a focus on smaller values in order to find models which are evaluated quickly. 

Taking this into account, the hyperparameter optimisation can be performed on the grid. In order to find competitive models, the configurations are rated according to the cost function
\begin{equation*}
    C=\sqrt{\bar t }\times(\bar \sigma +\sigma_{\sigma})
\end{equation*}
This means that the cost is the product of the square root of the mean training duration $\bar t$ and the  upper limit of the error in 84\% of the runs, calculated from the mean error $\bar \sigma$ plus the standard deviation of the error $\sigma_{\sigma}$. The reasoning behind the square root of the mean training is to take the cost of very small learning rates into account, as the precision could be also increased by sampling more points. The training time is here taken as a proxy of the evaluation time, as more complex models are both more costly to train and to sample from.

\Cref{tab:vardur} showed that there is a substantial spread in the improvement of \zunis relative to \textsc{VEGAS}. This becomes also clear from \cref{fig:madgraphviolin}. For the more easily trainable process $ e^- \mu \rightarrow e^- \mu$ via $Z$, the \zunis outperforms the benchmark virtually always, with a rather wide spread of the results. The other two process are, due to the presence of parton distribution functions, more challenging. These processes tend to have outliers with very high improvements, but also a significant fraction of runs which achieved no satisfying improvement. Nevertheless, the average improvement in comparison to \textsc {VEGAS} is substantial, and models which trained with under-average success can be filtered out after testing with a small set of evaluation points.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{performance/emmum_winners_loss_var.png}
    \includegraphics[width=0.45\textwidth]{performance/emmum_winners_loss_var_violin.png}
    \includegraphics[width=0.45\textwidth]{performance/ddx_winners_loss_var.png}
    \includegraphics[width=0.45\textwidth]{performance/ddx_winners_loss_var_violin.png}
    \includegraphics[width=0.45\textwidth]{performance/ucg_winners_loss_var.png}
    \includegraphics[width=0.45\textwidth]{performance/ucg_winners_loss_var_violin.png}
    \caption{The position of each of the trained models in the relative duration/relative variance plane (left) and the distribution of the relative variance (right) for $ e^- \mu \rightarrow e^- \mu$ via $Z$ (top),  $ d \bar d \rightarrow d \bar d$ via $Z$ (middle) and   $ u c \rightarrow u c g$ (bottom).}
    \label{fig:madgraphviolin}
\end{figure}



